Character-Oriented Design for Visual Data Storytelling

When telling a data story, an author has an intention they seek to convey to an audience. This intention can be of many forms such as to persuade, to educate, to inform, or even to entertain. In addition to expressing their intention, the story plot must balance being consumable and enjoyable while preserving scientific integrity. In data stories, numerous methods have been identified for constructing and presenting a plot. However, there is an opportunity to expand how we think and create the visual elements that present the story. Stories are brought to life by characters; often they are what make a story captivating, enjoyable, memorable, and facilitate following the plot until the end. Through the analysis of 160 existing data stories, we systematically investigate and identify distinguishable features of characters in data stories, and we illustrate how they feed into the broader concept of "character-oriented design". We identify the roles and visual representations data characters assume as well as the types of relationships these roles have with one another. We identify characteristics of antagonists as well as define conflict in data stories. We find the need for an identifiable central character that the audience latches on to in order to follow the narrative and identify their visual representations. We then illustrate "character-oriented design" by showing how to develop data characters with common data story plots. With this work, we present a framework for data characters derived from our analysis; we then offer our extension to the data storytelling process using character-oriented design. To access our supplemental materials please visit https://chaorientdesignds.github.io/

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> Sections/outdated/02_relatedworks.tex <==
% \section{Related Work}
% Character driven:
% To make it compelling you add a few outside forces
% Or a few characters and their interactions are the plot

\section{Storytelling in Visualization}
% The literature on methodologies for the design process for creating data-driven stories as well as techniques for communicating a narrative pull from a variety of domains such as journalism~\cite{segel2010narrative,stolper2016emerging,wangNarvis2019,chen2018supporting,wangDataShot2020,shi2020calliope}, comics~\cite{bach2018design}, and into media for data-videos~\cite{amini2015understanding,juddDoc2020,yang2022}.
% Within communicative visualization we have some understanding of how to utilize the power of narratives in conjunction with multitude of visualization design strategies~\cite{tong2018storytelling} to convey the author's intents. 
% However, there are still many challenges such as creating immersive data stories that illicit a connection to the intended message or offering a consistent way to guide people between story points (i.e., a through-line). 
% There is a wide body of literature in the visualization community that utilizes storytelling, where data storytelling and narrative visualization are two notable branches. 
Within visualization there is a large body of work that utilizes storytelling.
Data storytelling and narrative visualization are two notable branches. 
Recently, the literature contained in these branches were further organized into three groups~\cite{tong2018storytelling}.
The works are sorted based on whether they (1) address \textit{who are the main subjects involved} (authoring tools and audience),  (2) assess \textit{how stories are told} (narratives and transitions), or (3) consider \textit{why storytelling is effective for visualization} (memorability and interpretation).
% In a recent survey~\cite{tong2018storytelling}, the narrative visualization literature was organized into three groups.
% The first (1) details who are the main subjects involved in storytelling for visualization (authoring tools and audience), (2) how are stories told (narratives and transitions), and (3) why can we use storytelling for visualization (memorability and interpretation).
This paper seeks to contribute to  \textit{how stories are told} using a character-oriented design.
We find little has been done to address the design of data characters, since there is a current focus on creating and conveying the data story plot.
The general storytelling process~\cite{truby2008anatomy,field2005screenplay} considers both the plot and characters.
To better see the relation between the storyteller and the data storyteller, we organize data storytelling literature into three stages, as shown in~\autoref{fig:ds_process},  based on the storyteller's process: identification, organization, and presentation of the story.
In each of the three stages, we show how the narrative visualization and data storytelling literature address data story plot and the role of a character.

% ~\cite{tang2017extracting, demiralp2017foresight, cui2019text, dibia2019data2vis, srinivasan2018augmenting, wangDataShot2020,powerbi,narrativescience}
\subsection{Story Identification}
At the beginning of this stage, the data storyteller does not know what they want to discuss or share yet.
%However, unlike other storytelling mediums~\cite{field2005screenplay,truby2008anatomy}, data stories always consider ``non-alterable non-fiction''~\cite{isenberg2018immersive} and thus have less flexibility on creating the story. 
A set of events (or story pieces~\cite{lee2015more}), such as data facts or human insights, should be collected beforehand so that the author can figure out what to share and organize the story plot by ordering them via causality.
%Before a data story can begin it needs a set of events or story pieces~\cite{lee2015more}.
%These story pieces will later be ordered via causality to produce the story plot.
However, a consequent challenge is to create or identify these story pieces.


Some story pieces can be discovered through the analysis or the exploration of data, performed either by data analysts or the storyteller, while others are extracted from the discussion between data analysts and domain experts.
%For some instances, they are the result of working with others such as data analysts and domain experts whom will provide them with insights and findings.
%Other times, the storyteller takes on the role of the analyst and must go through the data to find something worth sharing.
Several tools have been developed to assist data exploration and help identify interesting findings~\cite{tang2017extracting, demiralp2017foresight, cui2019text, dibia2019data2vis}, while others~\cite{srinivasan2018augmenting, wangDataShot2020} aim to automate this process (i.e., insight generation).
%There are several works~\cite{bryan2016temporal,ren2017chartaccent,cui2019text,martinez2020data} on identifying or how to identify interesting findings via exploration of a dataset.
%This process is referred to as automatic insight extraction.
We have also noted efforts from the industry toward similar goals, such as Power BI~\cite{powerbi}, Lexio~\cite{narrativescience}, and Tableau.
%In addition, industry tools, such as Power BI~\cite{powerbi} and Tableau, 
% What is a plot point , how they associated with eachother, do these tools handle any of that, or do they just fiind POI;s
% There is the manual approach zzz, and the more hot area of automatic idenefication of POIS
%\textbf{TODO: brief summary and explanation of works that address automatic insight extraction}


In the context of characters and character design, this stage is not entirely applicable.
When discussing data characters, we are not concerned with the case of the story points being unknown to the author.
At the completion of this stage the author has acquired the story pieces that will inspire or lead them to determine what story they will tell. 
% However, as shown in Figure,  after the author has identified important data characters in the later stages, these characters can help better locate story pieces with a consistent message when the author revisit this stage.
Furthermore, it is only after identifying the story pieces,~\autoref{fig:ds_process}, that the data storyteller can start developing characters.
Although this manuscript does not focus on the identification stage, it is important to note the body of work that addresses it. 

\subsection{Story Organization}
Having a set of story pieces to report does not give a story.
Through their relationships with each other, they need to be sequenced into a story plot for presentation.
%These events need to be linked to each other and a story plot needs to be identified. 
If the author is unclear on the relationships and why the subject matter is worth presenting, the audience will feel similarly when consuming the story. 
It is in the organization stage that we determine the sequence
%order and sequence 
of story pieces and mold our story plot.
At the end of this stage, we should leave with a structured outline for our story.
Additionally, we also decide what genre~\cite{segel2010narrative} of the story will be and its setting~\cite{lee2015more} in this stage.
Several frameworks offer systematic ways to sequence a story plot for various genres~\cite{ojo2018patterns,segel2010narrative,yang2022,bach2018design, hullman2011visualization}.
% , or aimed to automate this process~\cite{hullman2013deeper, kim2017graphscape}.
Here we review the related literature on story plots from two aspects: the story structure and the communicative goal.
%The literature offers several frameworks~\cite{ojo2018patterns,segel2010narrative,yang2022,bach2018design} and methods~\cite{hullman2011visualization,hullman2013deeper} that can be utilized for this stage.
%gershon2001storytelling, kosara2013storytelling

% After going through the iterative process of identifying, analyzing, and deriving insights we arrive with a set of narrative events.
% Next, the author must organize and structure these events into a cohesive plot.
% They must also determine what type of story they are telling as to better assist them into understanding how these events relate to one another or what events should be omitted.

% Ordering & Organizing the narrative and events
%narrative rhetoric~\cite{hullman2011visualization}
%narrative sequencing~\cite{hullman2013deeper}

% Genres of a Narrative
% i.e., there are three types of story plot sequences?
There are a set of three narrative structures~\cite{segel2010narrative} for data storytelling, the drill-down, the martini glass, and the interactive slideshow, which have been widely used and heavily discussed in this space. %presentation
Recently, Yang et al.~\cite{yang2022} provide guidelines for applying Freytag's Pyramid, a narrative structure that has been widely used in film and literature, to data stories.
%
These structures are similar to what Truby~\cite{truby2008anatomy} describes as the story movement in the space of written storytelling.
Where he describes a set of patterns storytellers draw from nature to connect elements in some kind of sequence (e.g., linear, meanderings, spiral, and branching).
For data stories, narrative structure addresses story movement with a focus on the influence the audience has in controlling the pace of this movement.
% gives either the audience or the author more control in the pace of presenting a story plot.
The drill-down structure has an ability to present multiple story plots and even different stories, thus enabling the audience to explore the story.
Whereas, the other two often present a single linear story plot, which is easier for the author to maintain the plot consistency, and therefore has been the focus of automated reasoning~\cite{hullman2013deeper, kim2017graphscape}.
%The martini glass and the interactive slideshow are closer to how other forms of storytelling deliver plots, in a more linear sequence.

The author can narrow down their plot choice and ideal narrative structure by selecting a genre (or genres) that best fits their intention.
Segel and Heer~\cite{segel2010narrative} identify a set of genres: magazine, annotated chart~\cite{hullman2013contextifier,bryan2016temporal,ren2017chartaccent}, partitioned poster, flow chart, comic strip~\cite{bach2018design}, slide show~\cite{wangNarvis2019}, and film/video/animation~\cite{yang2022,amini2015understanding,bradbury2020documentary,amini2016authoring}.
Akin to other storytelling fields, these genres have the ability to be paired with each other.
Furthermore, many of these genres have been further developed, and methodologies and frameworks for using them have been offered. 
Refer to Tong et al.'s~\cite{tong2018storytelling} for more details

% Types of Data Plots
Adegboyega and Heravi~\cite{ojo2018patterns} identify seven types of plots from data stories.
% \begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
%     \item Refute claims.
%     \item Reveal unintended consequences.
%     \item Reveal information of personal interest.
%     \item Enable deeper understanding of a phenomenon.
%     \item Reveal anomalies and deficiencies in systems.
%     \item Reveal information about an entity in increasing levels of details.
%     \item Track changes in systems.
% \end{itemize}
% (1) refute claims, (2) reveal unintended consequences,(3) reveal information of personal interest, (4) enable deeper understanding of a phenomenon,(5) reveal anomalies and deficiencies in systems, (6) track changes in systems, and (7) to reveal information about an entity in increasing levels of details.
Their work provides a great jumping off point for character creation.
In Section 5.4 we describe generically how characters weave within these plots to convey the story.

% Thus, resulting in a loss of engagement.
% One factor could be a lack of a through-line to cohesively link sub-plots together and give a clear direction to the story.

% Storyboarding
Within the organization stage we also begin assessing which visual elements will best achieve our communicative goals and support telling the story plot.
We need to determine the importance of each visual element as well as what should be omitted ~\cite{hullman2011visualization}.
More importantly, we should note that having multiple story plots can lead to issues. 
Prior works~\cite{boy2015storytelling, dasu2020sea} illustrate how multiple sub-plots can lead to the audience struggling to comprehend what is presented and lose interest.
Possible explanations to this loss of engagement could be linked to the lack of an identifiable central character to reinforce the through-line.
Our work focuses on designing visual elements as data characters to help the author sequence the story pieces into a story with a clear message.
% which is agnostic to any narrative structures or types of plots, and applicable to any genres.

\subsection{Story Presentation}
At this stage, we have outlined our data story.
We know what we want to share, we have story pieces, we have organized them into a sequence, we have determined a structure, the genre, and now we are ready to realize our story.
Effective strategies for presentation include visual structuring, transitioning, annotating, and highlighting. 

% Visual Structuring
When presenting a story, several surveys~\cite{tong2018storytelling,segel2010narrative,stolper2016emerging} have thoroughly investigated the different presentation strategies depending on the genre (e.g., data comic, video, slide show, etc.). 
Stolper et al.~\cite{stolper2016emerging} identify effective techniques for presenting stories and map them to narrative structures~\cite{segel2010narrative} that Segel and Heer offered.
Additionally, an important part of storytelling is to smoothly transition~\cite{hullman2013deeper,kim2017graphscape,heer2007animated} between story pieces such that the audience can follow along.
% Stolper et al.~\cite{stolper2016emerging}, after reviewing relevant narrative visualization literature, identify what are applicable techniques for developing and presenting stories.
% Built upon the foundation that Segel and Heer~\cite{segel2010narrative} provided on narrative visualization and data storytelling, they further focus on the techniques and effective methods for presentation. 

% Annotations
Within visual data storytelling, there is a need to guide the audience directly to the story content and its importance. 
This is typically achieved via highlighting~\cite{segel2010narrative,stolper2016emerging}, annotating~\cite{hullman2011visualization,ren2017chartaccent}, or through the employment of text based methods~\cite{cui2019text,martinez2020data} for moving the story along.
Bryan et al.~\cite{bryan2016temporal} provide an authoring tool for apply annotations on top of existing visualization to serve a communicative need.
Hullman~\cite{hullman2011visualization} provides insights into how annotations should be curated, placement, and their narrative flow.

% There is some concerns in this process, as not all visualizations that are effective for exploratory tasks excel in explanatory tasks.
There are systems~\cite{wangNarvis2019,satyanarayan2014authoring,shi2020calliope} that merge in all three stages and provide authoring tools to generate data stories. 
These tools take an existing visualization as input, identify the events of interest, organize the events into a story plot, provide visual embellishments (e.g., annotations, highlight, etc.), and provide a means to export and share it.
Ellipsis~\cite{satyanarayan2014authoring} is a system for authoring narrative visualizations and provides a domain specific language that enables authors to apply stories to existing visualizations.
NarVis~\cite{wangNarvis2019} provides an interface assisting authors in explaining how to interpret their more complex visualizations via automatically generated tutorials.
From a storytelling perspective, NarVis's intent is to educate teachers and students on decoding a visualization.
Unlike other systems, this one not only takes an input visualization but also supports modifying the actual visualization rather than only supplementing with annotations.
Calliope~\cite{shi2020calliope} is another example, but unlike the others it takes a tabular dataset and automatically generates a story. 

Adapting existing visualizations for an explanatory purpose is clearly an important task.
% We can see from those works how relying only on annotations may not be enough, more effective communicative results can be achieved by adjusting the visualization to the explanatory need. 
From those works, we see that more effective communicative results can be achieved by adjusting the visualization to the explanatory need.
This may result in an entirely new visualization depending on the narrative goal.
We suggest further exploration into the design and selection of visual elements with a narrative goal.

% current works that "address character"
\subsection{Data Characters}
A data character would be the visual elements that are ``performing'' the data story~\cite{ma2012scientific}.
There are some direct references~\cite{ma2012scientific,shi2018meetingvis,zhao2015data} on the role a data character assumes; however, we all know you can not have a story without characters.
% However, all data storytelling address data characters, albeit indirectly, as you can not have a story without characters.
% We examine a set of works to draw properties for a data character.
When considering data characters, we are looking for visual entities with a narrative focus.
% The available works that assist us in further defining a data character fall into two groups: (1) (2)fundamental properties of a visualization (3) visual metaphor.
A data character would naturally take on rules of a visual encoding, the well established combination of marks and channels with their respective mappings to data.
It also needs properties that delve deeper into the communicative effort and that help the audience bridge the gap between the science and the story.
Thus, a foundation for the properties of a data character can be derived from works that address visualization design~\cite{shi2018meetingvis,morais2020showing,boy2017showing,stolper2016emerging,zhao2015data} and visual metaphors~\cite{risch2008role,petridis2019human,li2015metaphoric,cai2015applying,sallaberry2016contact,wang2015design,cruz2018process}.

% A set of work have addressed character-based or character-driven storytelling as well as touched on the role of characters in data storytelling.
Prior research have addressed character-based~\cite{cavazza2001narrative,cavazza2001characters} or character-driven storytelling~\cite{caiCharacterPlot,charles2001character}. 
Cai et al.~\cite{caiCharacterPlot} address the importance of character and plot driven storytelling and offers a hybrid system involving both types of approaches. 
Similarly, Cavazza et al.~\cite{charles2001character,cavazza2001narrative,cavazza2001characters} focused on character-driven stories and proposed an engine that model character behaviors.
Their work had a clear focus on automatic narrative generation, character's in all of these works are presented as either human or virtual agents.
These works focus on improving stories that are either rooted in traditional storytelling (e.g., not data-driven and allow for more creative freedoms of the author) or express the story content using virtual humanoid agents.
Data stories, often are not expressed using human or virtual agents and often utilize abstract representations.
They are also often rooted in non-alterable non-fiction constraining the storytelling process a bit more.
Our work contends that we should view and think of the abstract representations as characters similar to how prior research applies techniques to virtual agents.


To provide recent examples of what we consider an effective data character, we look to the popular storyline visualization~\cite{storyline2012,gove2021automatic,baumgartl2021}.
This visualization depicts an abstract encoding that represents the progress of an entity during a temporal period.
This character is something that draws on audience's attention and can be used as a through-line and an entry point into understanding change and growth of a single data-driven entity.
Storyline visualizations contain multiple storylines illustrating their relationships and how they change.
Other existing examples are visualizations with properties that make them more identifiable or personable, such as anthropographics~\cite{morais2020showing,boy2017showing}.
These representations were shown to be effective~\cite{boy2017showing} in creating an emotional connection with underlying content.
From these works, we can ascertain the importance of a character to be both central and identifiable for the audience.
However, it is unclear how to select which element should be central to the story and how the implications of this decision effect the story delivery.
Furthermore, other works allude to data character design implying that the visual abstraction assumes humanistic properties~\cite{morais2020showing,zhao2015data}. 
There is limited research that addresses the role of a data-character in data storytelling.
With character oriented design, we seek to demonstrate how all data-derived visual elements can be viewed as different types of characters.
Additionally, we present a framework for understanding the relationships between characters and the effects this has on the storytelling.

% The available works that assist us in further defining a data character fall into three groups, (1) visual metaphors~\cite{wang2015design,cai2015applying} (2) story-line visualizations~\cite{gove2021automatic,baumgartl2021}, and (3) storytelling frameworks~\cite{morais2020showing,boy2017showing,wangDataShot2020,shi2020calliope,wangNarvis2019,chen2018supporting,bach2018design}.
% literature visualizations~\cite{john2019visual}.
% These three groups address the roles of characters at different levels but showcase the importance and use of this concept.
% We offer a slight modification on the process to give character and the through-line of story more consideration.



% Roles characters can serve based on what can be applicable to narrative vis literature
% In recent research, we see that both anthropomorphic~\cite{ivanov2018exploration} and anthropograhpic~\cite{morais2020showing,boy2017showing} application in data visualization are effective in creating identifiable entities and eliciting some emotional connection with the content.


% What current organization of data character do we have?
% Lead off into proceeding sections: How can we organize this and do better?
% As it stands we are currently unclear what is a data character, is it an encoding, is it a visualization, is it a narrative agent? 
% The concern that arise is are these character as a casual result of the exploratory process.
% We find that visual elements with an explanatory and more specifically storytelling purpose should be designed with being the best fit character for a specific role in the plot.


% \textit{How are stories in visualization different from traditional storytelling? Are there implications from these differences? How does addressing characters benefit a data storyteller?}

% \subsubsection{Visual Metaphors}
Visual metaphors provide a desirable aesthetic to the viewers by employing a more familiar representation.
They tap into common structures and concepts people are familiar with and use them as bridges into the abstract and unfamiliar. 
Visual metaphors help viewers translate~\cite{risch2008role} abstract concepts into a more understandable form.
When thinking about character design a visual metaphor appears as a natural fit.
It creates a familiar mapping that the audience can use as an entry point in.
The audience learns how the visual metaphor behaves and what that means.
For example, Wang et al.~\cite{wang2015design} studied how users react to different personal visualization designs. They found that illustrative designs are the most well-balanced for relaying information and motivating data explorations.
Sallaberry et al.~\cite{sallaberry2016contact} employed a biological metaphor to effectively illustrate multiple relationships in a hierarchical dataset.
Cai et al.~\cite{cai2015applying} create a glyph that takes advantage of automatic and unconscious information processing in the pre-attentive stage to convey meaning to users.
Li et al.~\cite{li2015metaphoric} present a study on glyph based metaphors in information visualization and find it can improve users fluency of information processing.
% Fung et al.~\cite{fung2015visual} developed an egocentric visualization based a tree metaphor. 
% In a later design study~\cite{fung2016design}, they compared their organic visual metaphor against a set of visualizations and found that their visually attractive approach was the best for at-a-glance characterization of the data.


However, creating tight and applicable visual metaphors is difficult. 
It is dependent on audience familiarity with the base structure and that there even exists a parallel structure~\cite{petridis2019human}.  
This is not to say visual metaphors should not be used as characters; in fact, when applicable they should be.
% Rather visual metaphors are one example of a data character
% Rather, it is to treat character as a large concept.
Cox~\cite{cox2006metaphoric} offers a mapping of data-visualization to metaphors, arguing that every visualization is a metaphor of the data and should always be seen like one.
We use this argument to view characters as a metaphor for visualizations with a narrative purpose.
If we are telling a data story, a character is taking on the same role as a visual metaphor.
The differences are that it is not focused on a structural mapping between two entities or relying on the audience to have a prior understanding of one of the structures.
It is instead assuming the role of an entity with a narrative purpose.


% While evaluating the value of the visual metaphors, Risch~\cite{risch2008role} argued that the users understand visualizations through image schemas--structural patterns established in their childhood. 
% By employing familiar visual metaphors, we enable the user to interpret the data in terms of existing internal schemas.
% An alternative idea, which is the focus of this work, is to explain the abstract via representing concepts as metaphoric characters and how applying character design in the early stages of story creation can benefit the design process.


% \textit{How does thinking in terms of characters relate or address visual metaphors?}


% For the authors How details the techniques used to present the story including how to transitions between events within a story.
% Looking at the works they site that do this we see how to guide not necessarily how to construct the story.
% The current narrative devices and strategies are being evaluated and tested up on plot driven stories.
% There are currently no works where we examine characters in a visualization.
% A characters current role is to morph and contort to convey a plot within a a plot driven story.
% Although, this is a sufficient for telling some set of stories, there is more we can do with a character which we will discuss further.

% \subsection{The Plot-driven Design Space}
% The current state of storytelling in visualization is one of a plot driven design space.
% The techniques ideas and theories created over the last set of years are shown and applied upon stories with a fixed plot and how to best communicate that to an audience.


% \subsection{Semiotics}
% The construction of narration or narrative structures is a way of placing signs in a context.
% Thus, it is possible to interpret signs as determined by intentions and to link intentions and action with certain subjects who may have carried them out.

% To qualify as independent human action, Aristotle's three conditions must be fulfilled. These are expressed in the three modal auxillaries, wanting, knowing, and being able (will, knowledge, and ability). These elements are required for any action. Social imperatives which are tied to the aforementioned modals are: may, must, and should and there negatives (not).

==> Sections/outdated/05_case_studies.tex <==
\section{Case Study}
One use case for character-oriented design is as a means to frame the communicative relationships within data stories.
By doing so, we offer a \textbf{language} to discuss the effectiveness, relationships, and communicative precision of explanatory visualization.
The following case studies are to illustrate how this can be achieved, where we take several explanatory visualizations in a different context and show an alternative way to discuss either their strengths or weakness and open up to new conversations about these visualizations.
To further ground data characters we examine a set of four examples that touch on different types of ICC's, genres, number of story plots, and types of antagonistic forces.
We look at a data comic, a data video, a museum exhibit, and a visual analytic use case.
For each of these examples, we seek to answer the following:
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
    \item Who is the MC and what are their properties?
    \item Does the story have an ICC and is it the MC?
    \item Who are the SCs?
    \item What is the antagonist force and how does it introduce conflict?
    \item What is the relationship between the plot and the characters?
    \item What is the main theme, the through-line?
\end{itemize}
% Data comics (encodings/visual elements as ICC, lack of antagonist)
% Data videos (narrator as ICC)
% Award winning data stories (good example)
% Storyline visualization (visualization as ICC, visualization level)
% Sea of genes (lack of through-line, system level)



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/Case-1-Comic.pdf}
    \caption{Credit: Willikin Woolf~\cite{WillikinWoolf} and data comic gallery~\cite{datacomicgallery}. (a) original data comic (b) ``productivity'' is both the MC and ICC (c1) ``wage'' is a SC (c2) x-axis with year (c3) y-axis with percentage change (c4) line chart with the same colors as the MC and ``wage''.  (d) AF is a mysterious force causing the separation.}
    \label{fig:data_comic}
\end{figure}
\subsection{Data Comics -- ``Something’s wrong''}
Data comic~\cite{bach2018design} is a new and popular genre for presenting information effectively and was inspired by the visual language of comics.
To get a sense of the application of character design and their relationship we will examine a data comic ``Something’s wrong'' by Willikin Wolf~\cite{WillikinWoolf} featured on Benjamin Bach's data comic gallery~\cite{datacomicgallery}.
This story depicts the relationship between two characters.
There are two identifiable characters that are utilizing anthropomorphism.
The MC in this case,~\autoref{fig:data_comic}-b, is ``productivity''.
We can infer that MC's personal desire is to maintain a current happy relationship, as seen in~\autoref{fig:data_comic}-a panel 1, with the ``wage'' character.
% Properties of the MC are its color and  facial expressions. 
In this case, the ICC and MC are one and the same, since the focus is centered around the ``productivity'' character.
For example, in~\autoref{fig:data_comic}-a panel 3, we see the panel focuses on the despondent ``productivity'' character. 

The supporting characters are,~\autoref{fig:data_comic}-c1 to c4, wage, the x- and y-axis, and the chart.
The ``wage'' character appears to want to stay with the MC, as seen in panels 1--3.
Panel 4, gives us the additional SCs of the axis and the chart.
The axis helps us understand more about ``wage'' and ``productivity'' as they give the additional context of their percentage change when they were close together and then when they started to separate.
The colors of ``wage'' and ``productivity'' map accordingly. 

The antagonistic force, in this story, would be the reason behind this separation.
A force that at least on this page of the comic is not addressed or explained further.
The AF introduces conflict to the MC in the form of separation from ``wage''. 
The through-line between all these events is to explain the relationship between ``wage'' and ``productivity''.
A possible theme could be to persuade the audience into thinking that wage and productivity should not drift apart and have a linear relationship.

Determining the plot type~\cite{ojo2018patterns} of this story requires some reasoning.
Based on the sequencing between events, in this case, the panels, and how the characters act out the plot we learn that the separation was unexpected and the cause is unknown to the characters themselves.
Since it's difficult to clearly state the author's original intent, we can infer that the plot type is \textit{revealing unintended consequences}.
This leaves the audience with a possible desire to explore further or question why this separation happened, which could be the author's original intent for the story.

% What is the takeaway from this case study? Can this story be improved Do they use character well. What can they do better based on character mapping idk.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/Case-2-Video.pdf}
%     \caption{Credit: Gapminder~\cite{gapminder}. The ICC and the MC differ. (b) MC anthropograhic collection that represents a family  (c1) Professor Rosling is ICC, (c2) icon to represent death, (c3) each block represents one billion people. (d) The AF is a misunderstanding around population growth introducing conflict that poor families are the cause. The goal of the story is to illustrate how saving poor children can actually prevent overpopulation.}
%     \label{fig:data_video}
% \end{figure}
% \subsection{Data Videos -- ``Will saving poor children lead to overpopulation?'' }
% Next, we look at a story created by GapMinder~\cite{gapminder},~\autoref{fig:data_video}, that is in the genre data videos~\cite{amini2015understanding,amini2016authoring}, which are short data-driven motion graphics.
% % The next example is in the genre of data video .
% This story is upfront in its intentions in defining the plot.
% Namely, the plot is \textit{refuting the claim} of ``saving poor children leads to overpopulation.''
% Thus, the through-line in this story is to persuade the audience that the claim of ``saving poor children leads to overpopulation'' is false.
% Every character across every plot point is actively working to depict this through-line.

% The identifiable central character (ICC) of this story is the human, Professor Hans Rosling, as the video opens up with him introducing the story and stating the claim is false.
% However, in the context of a data story, Professor Rosling is not the main character.
% The MC would be the data physicalization of anthropographic elements, the humanlike icons.
% The properties of the MC are a collection of anthropograpic elements denoting a family. 
% We see in~\autoref{fig:data_video}-a two large icons representing parents and the smaller ones upfront representing children. 

% % In this story the story plot is to refute a claim.
% We look at the desires of the ICC (Professor Rosling) and the MC ( anthropographic families) and its relationship to the antagonistic force.
% The ICC's desire is to show that if we save poor children then we actually slow if not prevent over population rather than the contrary.
% He actively works to fulfill this desire based on both his narration and interactions with the other characters.
% For example, in~\autoref{fig:data_video}-a we can see him gesturing to the block highlighting his talking points.
% Now, the desire of the MC would be to ensure their family survives.

% The antagonistic force is the \textit{misunderstanding} that saving poor children results in overpopulation.
% The conflict introduced is an accusation that the data shows poor people have larger families and therefore they are directly responsible for overpopulation.
% The main character needs to overcome this conflict.
% Through the conflict resolution the outcome of the story is achieved.
% In this case, that outcome being a \textit{refute of the claim}.
% So we need a character who faces the conflict and changes resulting in a demonstration that by saving poor children we actually stave off over population.
% This is achieved through the MC in the data video.
% The ICC (Professor Rosling) actually assumes the role of a supporting character.

% The MC needs to persuade the audience that the death of poor children is not holding back population growth.
% The character of a poor family is presented, throughout the story we see what would happen if the children are saved and not left do die.
% We are shown how poor families suffer from high child mortality, and the largest population growth occurs where people are poor. 
% However, this is not the whole picture as parents in richer communities expect their children to survive, which is a factor for why they typically have fewer children.
% The supporting characters reveal how the over population issue can be addressed by saving poor children and how it can lessen the overall strain on population growth.

% ---------
% This needs to be re written since its directly taken from their website as the synopsis of the video.
% The poor families suffer from high child mortality, and the largest population growth occurs where people are poor. Parents in richer communities expect their children to survive, which is one of the reasons they decide to have fewer babies.
% Saving poor children is an important factor in ending both poverty and population growth.
% By revealing a motive for poor families to have more kids is to compensate for some of the children not surviving. An issue wealthier families do not deal with an is a factor in why those families are usually smaller
% Who is the main character? Professor Hans Rosling.
% Who are the supporting characters? and anthropographics.
% What is the antagonist force? The misunderstanding that ``Saving poor children leads to overpopulation''
% 	Are they addressed?
% What are the events. (a) (b) (c) (d)
% What is the plot? Refute claims ``Saving poor children leads to overpopulation.''
% What are the themes? To inform and persuade.
% What is the main theme aka through-line? To persuade the audience into understanding that saving poor children prevents overpopulation.
% \subsection{Visualization -- Storyline Visualization}
% Who is the main character?
% Who are the supporting characters?
% What is the antagonist force?
% 	Are they addressed?
% What are the events
% What is the plot?
% What are the themes?
% What is the main theme aka through-line?


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{/figures/Case-3-Exhibit.pdf}
    \caption{Credit: Sea of Genes~\cite{dasu2020sea}. (a) Museum exhibit containing a data-driven animation of a microbial community. (b) Three possible MC's that represent different microbes. (c1) side panel describing the scientists role and the data (c2) anthropomorphized annotations (c3) current relative time (c4) info card showing microbial gene expressions. (d) Antagonist interferes with the relationship between microbes and genes.}
    \label{fig:sog}
\end{figure}
\subsection{System -- Sea of Genes}
% Describe this story~\autoref{fig:sog}.
Sea of Genes~\cite{dasu2020sea} is a museum exhibit that is a combination of two genres (animation and annotated chart).
This exhibit, as documented, attempted to convey three story plots.
\begin{enumerate}[noitemsep,topsep=2pt,parsep=0pt,partopsep=0pt]
    \item Microbes interact with each other in a predictable daily rhythm.
    \item Genes turn on and off according to a daily rhythm.
    \item Scientists collect data about the genes of microbes.
\end{enumerate}
We can see a small issue that there is no obvious through-line between these three plots.
Two of them can be linked by genes, S2 and S3 , and another two by microbes, S1 and S2.
A possible through-line could be to inform the audience about how scientists collect data to evidence that microbes daily interactions are linked to their genes.
However, in their reflection~\cite{dasu2020sea} on the exhibit design the authors have two intentions to engage and inform the audience. 

The main character and the identifiable character in this story appear to be one and the same.
We see that we have three characters competing to be the MC,~\autoref{fig:sog}-b.
They have their own set of attributes (e.g., unique visual, animations, movement) and behaviors (e.g., making sugar, eating sugar, or infecting) that are dependent on the type of microbe.
The possible MC's are visual metaphors taking on some anthropomorphic attributes in the form of human-like annotations~(\autoref{fig:sog}-c2).
Their desire is to have a stable and sustainable community.

The antagonistic force in this story would be the \textit{misunderstanding} that microbes lack the sophistication to have a daily rhythm.
However, this doesn't capture the genetic portion of the story.
The conflict should arise between the microbes and their gene expressions.
Since, the S1--3 could be captured by that relationship.
The AF that instigates conflict in this story is unclear.
This story in a lot of ways lacks conflict.

When presented to an audience majority only received the first plot point.
Based on the evaluations, the other two had limited success.
There are a myriad of reasons as to why this story had communication issues, but we are interested in using characters to assess the story.
Most of the supporting characters either support S1 or S2.
One SC addresses S3, which is in the side panel~\autoref{fig:sog}-c1,
It is reasonable as to why S3 would not be of note to the audience as it is not a focus point of the MC's and is only addressed by one of many SCs.

So can we explain why S2 is not communicated using characters?
Well the MC's address genes, however, it is is not actively displayed.
To view the genetic information of a microbe requires an optional user interaction.
From the author's evaluation it appears the audience did not know how to interact with the MCs (animation). 
% Furthermore, whether the few that did may not have made the association between the panels displaying genetic information,~\autoref{fig:sog}e 1, and the ring that would appear,~\autoref{fig:sog}e 2.
In terms of characters, there is a link between the MC and the genetic based story of S2, however it is not emphasized and relies on an optional interaction to access.
The only story that is constantly put forth and actively displayed to the audience is that there is an animated microbial community that exists through out the day and is always doing something.
This overall story plot type seems to be a combination of a \textit{deeper understanding of something} as well as \textit{reveal information of personal interest}.


% Our character has its base physical attributes and properties as well as actions it performs.
% Let us use Procholoroccus as an example.
% This microbe has a physical description of what it looks like as well as what actions it performs and when it does.
% We also know what genes are being expressed when the action is performed so our character should illustrate this is some capacity.
% It should illustrate that the action being exhibited was triggered because a set of genes were expressed.
% We also need to express the action that is being performed.
% We apply this design to each of our characters and as a result we get the following.
% We now introduce each character to our audience such that they gain an understanding about each one.
% Then we show how each character behaves when it comes into contact with another.
% If we portray this a static comic or illustration we see this.
% There are a variety of ways that this could be presented (e.g. Animation, Video, Comic).
% Selecting the medium for how it should be presented depends on the context~\cite{lee2015more}.

\subsection{Use Case -- Visual Analytics of Air Pollution Data}
Use cases are commonly used in the application papers to demonstrate the applicability of a visualization system.
The plot type of these type of stories are a~\textit{deeper understanding of something}, specifically a system. 
%Case studies are commonly used in the visualization system or application papers to demonstrate the applicability of a system.
%These case studies can be data stories as 
% Need to motivate more on why we are using the case study as one example and how relating them to data stories helps?
We include one use case from a visual analytic paper~\cite{kuo2022machine} that introduces a system consisting of coordinated interactive visualizations to support domain specific analysis.
% This is one common system setting in the visualization community.
% Shrink down the following if no space.
For context, the author develops a methodology to decompose the air pollution data into three aspects: what (pollution sources), where (monitoring stations), and when (days), and considers a pollution event to contain the three aforementioned properties. 
Several interactive visualizations are designed to support analyzing each of the three aspects as well as their combinations.
%The coordination then helps the user flexibly transition between different aspects based on the analysis needs.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{/figures/Case-4-VA.pdf}
    \caption{Credit: Kuo et al.~\cite{kuo2022machine}. (a) An annotated use case used in the paper that shows the process of revealing a hidden air pollution event in 5 steps (a1-a5). (b) The MC is the introduced visual analytic system. (c1) The paper author is the ICC as a narrator agent. (c2, c3) SCs that help reveal the properties of an event before encountering the conflict. (c4-6) SCs that help the MC overcome the conflict. (d) The antagonist force along with the conflict appears in a3.}
    \label{fig:va_case}
\end{figure}

As shown in~\autoref{fig:va_case}-a, the author presents five snippets in this use case that can be expressed as the following story pieces: 
%As the last piece (f) is included to illustrate another capability of the system, we only consider the first 5 pieces (a-e) as they already describe a complete story.
% The plot points of this use case:
% While (d) provides a detailed examination of the data (i.e., the observation values of air pollutants), 
% Through interactions,  (e)
\begin{enumerate}[noitemsep,topsep=2pt,parsep=0pt,partopsep=0pt]
    \item The high green bars in (a1) indicate that many pollution sources characterize the stations in the green cluster. This can motivate the user to pursue understanding when would these sources have strong influences on these locations;
    \item The higher green line of pollution source D with annotations in (a2) suggest source D may affect the stations in the green cluster during the annotated time period;
    \item For the stations in the green cluster (a3) , the user only finds an observed anomaly at one time point.  % rather than the suggested period;
    \item The user observes from (a4) that source D has the highest contribution at one station within the suggested period;
    \item  From (a5), the user now understands that source D is characterized by the annotated heavy metals. With external information, the author concludes the inferred pollution event through texts.
\end{enumerate}

% While not illustrated in the figure, with the external materials, the author explained that source D is highly related to joss paper burning, which plays an important role in the Qingming festival.

The through-line of these story pieces is to explain the effectiveness of the system for supporting domain specific analysis.
The author of the use case is the ICC as they take on the role of a narrative agent and guide the audience. % through this use case through plain texts.
Our MC is the system and it has a desire to show a pollution event.
The ICC's desire is to showcase the strengths of the MC by revealing a hidden air pollution event. % using the system.
Thereby, making the ICC an SC.
As for the antagonistic force, it can be misunderstandings about the pollution event, such as other causes or ambiguity in either the data or the visualization, it creates obstacles for the MC. 
%One AF appears in the third 

In the first two story pieces, the ICC highlights two visualization components in the MC to indicate the potential presence of a pollution event in a region, by revealing two of the three properties (what and when).
The green bar in (a1) and the annotation in (a2) can then be considered as two SCs, as shown in~\autoref{fig:va_case}-c2 and c3.
In the third story piece, the ICC unpacks properties of the MC, in an attempt to reveal the where property.
However, the observation values reveal contradicting information about the when property resulting in an obstacle.
% The antagonistic force then can be identified as the grey lines that record the observation values of pollutants.
% Utilizing the methodology introduced in the paper,
To help the MC overcome this obstacle, the author presents a supporting evidence (\autoref{fig:va_case}-c4) that clarifies the three properties in a pollution event.
In the last story piece, the author utilizes the information provided by a visual component along with the official reports (\autoref{fig:va_case}-c5 and c6) to further dispute the obstacles introduced by the AF. 
With the help of the three SCs (the black lines, the annotation, and the explanation texts) introduced in the last two story pieces, the MC overcomes the obstacles and reveals the air pollution event.



% ----------------------

%The conflict introduced lies in the third story piece
% Particularly, how this event consists of three properties (i.e., contributing pollution source, location, and time) and 
% For more details, please refer to the paper.


% \textbf{TODO: Yun-Hsin make this inline with the above, demonstrate how the telling of effectiveness of the system is played out through showing the strengths of the system, how the author tries to support building up the system to be effective at the tasks, how AF tries to expose and either is successful or not and how the MC (system) responds to these conflicts in the context of a case study. The resolution of all of this should arrive at the point the author wanted to make with the case study in the first place.}

%How this is played out in the story is by the ICC first introducing us to the MC.


%The ICC explains that source D is highly related to joss paper burning, which plays an important role in the Qingming festival.
%Official reports also confirmed that there were pollution events happen during the suggested time period due to this forthcoming festival.
% As the author leads the audience to go through the story via plain texts with annotations in the figure, the author is identified as the ICC, where the desire is to reveal a hidden air pollution event using the system.
%Other supporting characters (e.g., the visual encodings, such as bars and lines in~\autoref{fig:va_case}C) help reveal the information of a potential pollution event by serving as entry points, since they depict 
%the relationships among the properties of a pollution event (e.g., ~\autoref{fig:va_case}A-a shows the relationship between locations and pollution sources).
%the relationships among different aspects (i.e., the properties of a pollution event).
%The conflict lies in the third story piece that we only see a potential time point rather than a time period revealed by the SCs.





















%The antagonistic force (AC) is the observation values (grey lines in (d)) of the stations, where the y-axis in (d) can be considered to be the SC of the AC.

% While we are able to address these elements with character-oriented design, we have to note that the genre is why the audience is not lost in the story.
%In the scenario where the user is using the system, we lost the author as the ICC.
%Although other characters remain in their roles, we cannot identify the MC, the air pollution event, as the ICC.
%Since in every story piece, only part of the MC's properties are brought out through the relationships among the SCs.
%We recommend incorporating a visual encoding for the pollution event as the ICC, such as a glyph that can encompass the three properties, so that the user can follow along to explore the system and perform analysis. 

%where the story still delivers the author's message that the system supports the domain specific analysis better and thus achieves the communicative goal.
%However, if the genre is changed from plain texts to data videos or the scenario that the user is using a web application

%What can make this story better: Alternative visualization design that utilizes the visual encoding for a pollution event, potentially a glyph so that we can incorporate the three properties of an event together.

%Who is the main character? (??)
%Who are the supporting characters? The encodings of pollution sources, the clusters, the aggregated contribution lines, the observation lines, the contribution lines per station... a lot of them.
%What is the antagonist force? The observed PM2.5 values of other stations indicate that the event may only happened.
%Are they addressed?

%What are the events? Each of the views, a-e, (f).
%What is the plot? a, c, d, e, b, (f), sequenced by the characters' relationships.
%What is the plot type? To reveal information about an entity in increasing levels of details.
%What are the themes? To explain to the air pollution analysis experts that the designed visual analytic system better support their analysis.
%What is the main theme aka through-line? A pollution event happens at a location, during a time period, caused by a pollution source. Or a higher level, the designed visual analytic system better support the analysis.

%In terms of paper, this works because the ICC is the author. In the system, it can be better as only part of the ICC (i.e., the event) properties are revealed at the same time.





==> Sections/outdated/06_analysis.tex <==

\section{Analysis}
 To better understand the nature of data characters, the forms that they assume, and their behavior in data storytelling we created a corpus of  ~130 data stories by merging several other corpora and updating them with some newer stories [site above 1–7]. The merged corpus size was reduced based on repeats and any stories that were no longer accessible (i.e., required adobe flash or no longer online). 

We further filtered down the set to primarily visual stories. That is the content of the story and core messages were communicated via data-driven visualizations, animations, or video rather than heavily dependent on multiple paragraphs of text. The latter case refers to stories where the visualizations serve as an annotation or figures and are not the driving narrative force. 
Based on the coding framework, two researchers independently coded the corpus. We met for three sessions to compare our codes and discuss mismatches until we reached a 100\% consensus. \yunhsin{Throughout the process, we identified a few limited dimensions in the codebook and consequently edit the codebook to address the limitations, e.g., we include a new type, real-world photos, for ICCs. The finalized codebook is presented in~\autoref{tab: codebook}.}

It is common for data stories to lack a visual entity that is readily identifiable and central to the narrative. Often data story stories contain many encodings, charts, and graphics to tell their story. However, in these scenarios, the through-line or unifying concept is primarily conveyed through the accompanying text. In these stories, the visualizations and visuals serve a secondary role in the narrative. 


From our analysis, we identify distinguishable features of data characters and the roles they serve and present a design space for designing data characters.
Additionally, we derive that the role visual elements and visualizations serve in data storytelling fall into two states: (1) \textit{given an existing visualization, how can we adapt it to emphasize and explain a finding\cite{srinivasan2018augmenting}} and (2) \textit{given a finding, how can we visualize it~\cite{shi2020calliope}}. 
Both states share the goal of data storytelling; however,  they both present two different starting points for what we view as characters.
The former has an existing character that will be developed and altered to depict the plot, whereas the latter starts from scratch.
Plot points are always conveyed through the characters' actions and interactions within the setting.
From the extant literature,  we have an understanding of identifying, organizing, and presenting the story plot.
However, we still have challenges in data storytelling and areas to improve upon that a character-oriented approach could address.
We still need to work on methods for maintaining and presenting the connections between our story pieces (i.e., through-line) as well as offer a direction on how to elicit an emotional connection to the stories we tell.
Designing the story pieces in terms of characters facilitates seeing and tracking continuity in a story. 
% As stated, we are interested in leaning into character design to assist the author in creating richer stories and thinking about visual elements from a character-oriented space.






==> Sections/temp.tex <==
\begin{tabular}{p{0.01\textwidth}>{\raggedright}p{0.175\textwidth}>{\raggedright}p{0.33\textwidth}p{0.37\textwidth}}
    \toprule
    
    \textbf{Character Terminology} & 
    \textbf{Description} \\
    %\arrayrulecolor{black!30} \midrule
    
    %\multicolumn{2}{p{1.5625in}}{\textbf{Fundamental Concepts}} &  &  \\
    &
    \textbf{Character} & A visual entity that influences itself and others and serves a narrative purpose. \\
  
    Desire & 
    The rationale that motivates a character's actions toward a goal \\
    
    Conflict &
    Arises when an entity attempts to accomplish something against the obstacles in its way. The pressure that is applied to the MC forces change. \\
    
    Archetypes &
    Patterns within an entity; the roles they play are essential in how they interact with others. \\
    
    \tabIndent Main Character (MC) &
    Has the central problem and drives the action in an attempt to solve the problem. They have a personal desire that they seek to attain, but forces prevent them. \\
    
    \tabIndent Supporting Character (SC) &
    This character type complements either the MC or AC. They provide a means for the audience to see more depth about the MC or AC. An SC's desire can align with either the AC or MC, but will not go against it. \\
    
    \tabIndent Antagonist (AC) &
    Seeks to prevent the hero from reaching their desire. They come into conflict, and through working out the conflict between the two the story plays out. They can be a character or an external force. \\
     
  
   %\midrule
   \bottomrule

\end{tabular}

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

